Morphologic for knowledge dynamics: revision, fusion, abduction

Several tasks in artificial intelligence require to be able to find models about knowledge dynamics. They include belief revision, fusion and belief merging, and abduction. In this paper we exploit the algebraic framework of mathematical morphology in the context of propositional logic, and define operations such as dilation or erosion of a set of formulas. We derive concrete operators, based on a semantic approach, that have an intuitive interpretation and that are formally well behaved, to perform revision, fusion and abduction. Computation and tractability are addressed, and simple examples illustrate the typical results that can be obtained.

==> conclusion-essai.tex <==
\section{Final remarks and perspectives}
\label{sec:conclu}

We have given the fundamental concepts and techniques in mathematical morphology, and have shown how to interpret these techniques
in terms of mathematical logic, namely in propositional logic. This connection has originated a new domain called morphologic. We have
used dilation operators in order to define belief revision operators and belief merging operators.

We have shown that we
can find some operators defined in the literature when the dilation operators come from a distance. Moreover we have extended
the class of belief revision operators and the class of belief merging operators by using a larger class of operators, in particular having the extensivity and exhaustivity properties.

A similar work has been done using contraction operators. These operators are used in two ways in order to define explanatory relations.
It is interesting to note that the use of different structuring elements is determinant in the way the information is structured.
The examples in Section~\ref{abdu:examples} point out in a clear way this phenomenon.

Under the assumption that the geometry comes from the Hamming distance between interpretations, 
we have shown how to compute dilation, erosion, last erosion, ultimate erosion, opening and
skeleton operators over formulas. These calculations constitute the basis of our applications to 
different tasks in knowledge representation.

We have proven that our general operators of revision and fusion are well behaved, in particular they satisfy the AGM postulates and the postulates
of integrity constraints belief merging. We have also proven that the explanatory relations defined using morphologic satisfied suitable structural properties. 

Potential extensions would be to analyze how minimality criteria for could be expressed in the proposed framework, as the ones proposed for abduction~\cite{bienvenu2008,eiter1995,halland2012}, revision for Horn clauses~\cite{DP11,DP15,ZPZ13} or for description logics~\cite{ARXIV,QLB06,QY08,RW09,RW10,WWT10}, or more generally for institutions~\cite{AABH15} and satisfaction systems~\cite{MA:AIJ-17}.

One interesting feature that is worth to remark is the fact that morphologic allows us to give an ordered structure to the pieces of information.
That is, it allows having preferences over the formulas. It is exploited by the morphological total pre-order defined by Equation~\ref{order3}. Note that these preferences
depend on the structuring element used for defining dilations and erosions. 

Finally, our approach provides a reusable framework for performing numerous operations on formulas, and includes computational and axiomatic building blocks, to be applied in different reasoning problems.

Future work will aim to apply the tools of morphologic in order to explain multiple observations and for putting dynamics in the explanatory process. We also expect to treat mediation process using the tools developed in this work.




%
%\fbox{TO DO:}
%\begin{itemize}
%\item several domains where the proposed definitions and results could be useful (briefly), which could be selected from the text below
%\end{itemize}
%
%
%\fbox{List of potential examples discussed previously (some of them could be kept?):}
%
%\begin{itemize}
%
%\item ``cube'': simple example with 3 variables, to illustrate the effect of the proposed operators. But too small to be a convincing applicative example.
%
%    {\em  I think there is in the draft two kinds of examples. The ones illustrating basic concepts (dilation, erosion, etc). Perhaps for this purpose the cube is good. The others examples deals with the
%    illustration of  pertinence of one operator. This is  the spirit of the political party's example below.
%
%    We have to find appropriated examples for illustrating \begin{enumerate}
%    \item revision,
%    \item fusion,
%    \item abduction,
%    \item generalized revision and abduction (the points which are in section 6 for the moment),
%    \item explanations of multiple observations (I think we cut the paper here. The morphological nature of mediation it seems to me very different... To discuss
%    )
%    \item mediation (???),
%     \item juxtaposition (???, work in progress)
%    \end{enumerate}}
%
%
%\item ECAI example:
%Suppose $X$ and $Y$ represent the political agenda of the Labor
%Party and the Green Party, respectively. They would like to find
%an agreement in order to present a common platform for the next
%elections. As it usually happens, there are several leanings in
%each of the two parties. In order to simplify, suppose there are
%two leanings in each party, the left and central. Their positions
%about ten parameters are encoded by worlds. The parameters are the
%following: nationalization of big private companies; increasing
%the taxes for the rich people; reducing the taxes for the poor
%people; increasing the budget of public health; increasing the
%budget for public education; creating a subvention for the
%unemployed persons; increasing the budget of research programs;
%reducing the subsidies for the big agriculture exploitations;
%creating subsidies for organic agriculture; fostering the public
%transports. The encoding is made in the following manner:
%$X=\{w_1,w_2\}$, $Y=\{w_1,w_3\}$, where
%$w_1=(1,1,1,1,1,1,1,1,1,1)$ is the encoding of the left wing in
%both parties, the central wing in the Labor Party is encoded by
%$w_2=(0,0,0,1,1,1,1,0,0,0)$ and the central wing in the Green
%Party by $w_3=(0,0,0,0,0,0,0,1,1,1)$. If the policy adopted for
%merging these leanings is a classical fusion, in which the result
%is $\{w_1\}$ (the intersection of both groups), they run the
%risk of the splitting of both political parties. Thus they have to
%adopt a different  policy in order to reach an agreement more fair
%to all leanings.
%
%\begin{center}
%\begin{tabular}{ccccccccccc}
%$w_1$: & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
%$w_2$: & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 0 & 0 & 0 \\
%$w_3$: & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 1 \\
%\end{tabular}
%\end{center}
%
%$X = \{ w_1, w_2 \}$, $Y = \{ w_1, w_3 \}$ -- Classical fusion $\Rightarrow \{ w_1 \}$
%
%
%Why not:
%\begin{center}
%\begin{tabular}{ccccccccccc}
%$w$: & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\
%\end{tabular} ?
%\end{center}
%
%\includegraphics[width=10cm]{Figures/notFairInters.png}
%
%Fusion: the same result in both cases. Fusion then explanation: also the same result in both cases. Favors the agents with the more restricted preferences.
%
%Mediation: the result would be pushed towards the right of the figure. Favors the agents with the more flexibility in their preferences.
%
%Explanation then fusion: we take the most central part of each set, and then try to find a median solution between these explanations. Would provide also a different result in each case.
%
%The most central part provides a clear positioning of the representative of a group who will discuss in an assembly.
%
%\item Importance of available ``resources'': if they are low, fusion might be better; if they are larger, juxtaposition would be better. Ex: bying books in a lab.
%
%\item Music example: an agent expresses his preferences about music. He is interested in different types of music and expresses his preferences in a disjunctive form. For instance he is interested in traditional Indian music, in romantic German music and in contemporary western music. If we want to find ``typical examples'' of his preferences, it would not make sense to choose only one type of music, and we would prefer to propose examples in each type.
%
%In this example it is not interesting to consider the disjunction of all preferences as one set. It is more meaningful to consider the ``juxtaposition'' of the three types of preferences. The explanations would then also be expressed as a juxtaposition. {\em This is  a very natural way of considering these different observations.
%Grosso modo it is the n-vector of these observations. Then it is interesting to find the explanation also in terms of juxtaposition.} Refers to multiple observations.
%
%
%The ultimate erosion could also be a useful tool in such cases.

%
%\item Similar example with food: someone can be interested both in ``grands chefs'' restaurants and in small popular ``boui boui''.
%
%\item J\'er\^ome's example: preference-based search, e-commerce
%
%\item Choice of a city for a conference: each $\alpha_i$ represents a set of proposals. The choice criterion is a distance to $\Sigma$ (easy access from the tain station, conference facilities, cultural environment, etc.). We choose at least one city in each $\alpha_i$. If a city has been chosen in $\alpha_i$, all cities in $\alpha_j$ which are not farther from $\Sigma$ than this city could be chosen as well since they satisfy the criterion too.
%This example could explain why the same dilation should be performed in the case of juxtaposition.
%
%\item Geometrical / spatial example: Let us consider a mobile robot moving in a museum, i.e. an environment with fragile objects. The robot should not touch the museum objects, and even stay as far as possible from them. Possible states are then $(\cup_i O_i)^c \equiv \llbracket \varphi \rrbracket$, where $O_i$ are the fragile objects + some graph structure representing the actions allowing the robot to move from one place to another one (e.g. from a place $x$, the robot can move only along the edges issued from $x$ in the graph of places). Safest place for the robot: $\varepsilon_\ell (\varphi)$.
%
%\end{itemize}
%

